Giving RSEs a Larger Stage through the Better Scientific Software Fellowship

The Better Scientific Software Fellowship (BSSwF) was launched in 2018 to foster and promote practices, processes, and tools to improve developer productivity and software sustainability of scientific codes. BSSwF's vision is to grow the community with practitioners, leaders, mentors, and consultants to increase the visibility of scientific software production and sustainability. Over the last five years, many fellowship recipients and honorable mentions have identified as research software engineers (RSEs). This paper provides case studies from several of the program's participants to illustrate some of the diverse ways BSSwF has benefited both the RSE and scientific communities. In an environment where the contributions of RSEs are too often undervalued, we believe that programs such as BSSwF can be a valuable means to recognize and encourage community members to step outside of their regular commitments and expand on their work, collaborations and ideas for a larger audience.

==> bios.tex <==
\begin{IEEEbiography}{Daniel S. Katz,}{\,}
is Chief Scientist at the National Center for Supercomputing Applications (NCSA) and Research Associate Professor in Computer Science, Electrical and Computer Engineering, and the School of Information Sciences (iSchool) at the University of Illinois Urbana-Champaign.
Katz received the B.S., M.S., and Ph.D degrees in Electrical Engineering from Northwestern University in 1988, 1990, and 1994, respectively.
His interest is in the development and use of advanced cyberinfrastructure to solve challenging problems at multiple scales, including applications, algorithms, fault tolerance, and programming in parallel and distributed computing, as well as policy issues such as citation and credit mechanisms and practices associated with software and data, organization and community practices for collaboration, and career paths for computing researchers.
He is a co-founder and current Associate Editor-in-Chief of the Journal of Open Source Software, co-founder of the US Research Software Engineer Association (US-RSE), and co-founder and steering committee chair of the Research Software Alliance (ReSA).
Contact him at d.katz@ieee.org.
\end{IEEEbiography}

\begin{IEEEbiography}{Sarah E. Bratt,}{\,}
Dr. Sarah Bratt, PhD, is an Assistant Professor at the University of Arizona School of Information (iSchool). She holds a B.S. in Philosophy from Ithaca College and M.S. in Library and Information Science with a Data Science certificate from Syracuse University. Her research lies at the intersection of scholarly communication, research data management, and science of science. The overarching goal of her research is to understand and design for long-term research data sustainability and actionable science policy. Her research has been published in Quantitative Science Studies (QSS), Journal of Informetrics, and Scientometrics. She was a research Fellow at the Laboratory of Innovation Science at Harvard (LISH) and a Fellow at the iSchool Inclusion Institute (i3) and received multiple awards including the Masters’ prize in Library \& Information Science at Syracuse University and honorable mention as a 2022 Better Scientific Software (BSSw) Fellow. Dr. Bratt is a member of the ACM and IEEE Computer Society. Contact her at sebratt@arizona.edu.
\end{IEEEbiography}

\begin{IEEEbiography}{Damian Rouson,}{\,}  Damian Rouson is a Staff Scientist and Group Lead for the Computer Languages and Systems Software Group at Berkeley Lab.  He holds M.S. and Ph.D. degrees from Stanford University, a B.S. from Howard University, and a Professional Engineer license in the State of California, all in Mechanical Engineering.  His research interests include software archaeology, programming paradigms and patterns, parallel runtime libraries and solvers, applications of AI to high-performance computing, and turbulence in classical, quantum and magnetohydrodynamic media. He founded and leads Archaeologic Inc. and Sourcery Institute. He was the lead author on the textbook \emph{Scientific Software Design: The Object-Oriented Way} (Cambridge University Press, 2011) and has taught related courses at the University of Cyprus and Stanford University and short courses in over 30 other venues. He serves on the Editorial Board of \emph{CiSE}. Contact him at rouson@lbl.gov.
\end{IEEEbiography}

\begin{IEEEbiography}{Ritu Arora,}{\,}  Ritu Arora serves the University of Texas at San Antonio as the Assistant Vice President of Research Computing. She holds Ph.D. degree from the University of Alabama at Birmingham in Computer and Information Science. Her areas of research and expertise include high-performance computing, cloud computing, large-scale data management, and advanced software engineering. She can be contacted at ritu.arora@utsa.edu.
\end{IEEEbiography}

